An Empirical Study on the Characteristics of Database Access Bugs in Java Applications

Database-backed applications rely on the database access code to interact with the underlying database management systems (DBMSs). Although many prior studies aim at database access issues like SQL anti-patterns or SQL code smells, there is a lack of study of database access bugs during the maintenance of database-backed applications. In this paper, we empirically investigate 423 database access bugs collected from seven large-scale Java open source applications that use relational database management systems (e.g., MySQL or PostgreSQL). We study the characteristics (e.g., occurrence and root causes) of the bugs by manually examining the bug reports and commit histories. We find that the number of reported database and non-database access bugs share a similar trend but their modified files in bug fixing commits are different. Additionally, we generalize categories of the root causes of database access bugs, containing five main categories (SQL queries, Schema, API, Configuration, SQL query result) and 25 unique root causes. We find that the bugs pertaining to SQL queries, Schema, and API cover 84.2% of database access bugs across all studied applications. In particular, SQL queries bug (54%) and API bug (38.7%) are the most frequent issues when using JDBC and Hibernate, respectively. Finally, we provide a discussion on the implications of our findings for developers and researchers.

==> texFiles/rq2_old.tex <==
\hypertarget{rq2}{}
\subsection{RQ2: Where are database access bugs introduced?} 
\label{rq:rq2}

\peter{let's just keep Table~\ref{tab:issues_unique_files}. Move Table~\ref{tab:issues_unique_files} and its discussion to the end of RQ1. }\wei{Done}

\phead{Motivation.}
In this research, we want to know where database access bugs occur in the source code by studying the characteristics of commit source code files for database access bugs. Understanding of the characteristics of commit source code files may help developers narrow the occurrence place of potential database access bugs and further locate and fix them with fewer efforts.

\phead{Approach.}
We extract commit files for reported bugs and calculate the intersection on the collection of database access bugs and non database access bugs. We also study how many commit files for database access bugs call the database access APIs or contain the entity class.

%\phead{Results.}
%Table \ref{tab:issues_unique_files} summarizes the count of unique commit files for database access bugs and non database access bugs. The small count of intersection on the collection of database access bugs and non database access bugs indicates that they occur in different set of source code files. For the database access bugs, we examine the commit files to determine whether the commit files call the database access API or contain the entity class. Table \ref{tab:percentage_database_access} shows the percentage of unique commit files  which contain the entity class or call the database access API for database access bugs. We find that, around 20\% of all commit files for for database access bugs the database directly. 
%
%\rqbox{We find that database access bugs occur in some specific source code files compared to non database access bugs. Around 20\% of these specific source code files call database access APIs directly.}

%In order to study the characteristics of source code files where database access bugs are introduced, we study the characteristics of commit files for issues.
%We first extract all commits for each issue report and take the files changed in the commit as place where corresponding issue occurs.
%We also want to study the characteristics of committed files for database access bugs by examining which Java source code files are committed. 

% RQ1 studies the evolution history of database-related issues and shows the trend of issues occurrence. Furthermore, if the occurrence place range of database-related issues can be narrowed, they can be located and fixed with fewer efforts.

%The first step towards understanding database-related issues is to find out how they manifest themselves. In this research question, we evaluate database-related issues on several metrics. For example, we study what types of these issues: errors/bugs/defects/performance/. We study how many these issues are related to Java source code/configuration/SQL query. We also study where issues come from in the source code files (e.g. the database access layer or others). Knowing these characteristics might help developers prioritize their efforts when identifying and locating database-related issues. An comprehensive understanding of database-related issues also inspire future research on them. (In a word, this RQ focus on the characteristics of database-related issues themselves. The introducing and fixing practices from developers are also considered as characteristics of database-related issues. For example, the fix duration time is also one feature ot issues.)

%First, we compare the commit source code files between database-related issues and non database-related issues are introduced. Table \ref{tab:issues_metric} shows the metric results (i.e., LOC modified and Files modified) for per issue while Table \ref{tab:commits_metric} shows the metric results (i.e., LOC modified and Files modified) for per commit. There is no significant for commit source code difference between database-related issues and non database-related issues as most of the $p$-value is greater than 0.05 under the hypothesis H: DBIssue $\neq$ NDBIssue.
% we calculate the percentage of commit files which call the database access API or contain the entity class.  
% Last, we study how many commit files of database-related issues call the database access APIs. We calculate the percentage of entity class files and database access class files in all commit files by examining the source code of commit files.

%Then, we use entropy to measure the scatter of commits between  database-related and non database-related issues. The scatter of occurrence place indicates if they only change some files or if they need to modify other files too for database-related issues. The entropy is defined as:
%\begin{equation}
%	H(commit) = \frac{-\sum_{i=1}^{n} p(File_i) * \ln p(File_i)}{\ln n} 
%\end{equation}
%where $ n $ represents the total number of files in a commit $Commit$, and $ H(Commit) $ is the entropy value of the commit. $p(File_{i})$ is defined as the number of lines changed in $File_{i}$ over the total number of lines changed in every file of that commit. $ H(Commit) $ ranges between 0 to 1, where the larger the value more complex the distribution. For example, if we modify three files A (modify 1 line), B (modify 1 line), and C (modify 3 lines), then p(A) will be $\frac{1}{5}$ (i.e., $\frac{1}{1+1+3}$ ). Specifically, when $ n $ equals to 1, the entropy value is defined as 0.

%Persistent object classes map to database tables and database access classes manipulate database directly. Hence, they may be prone to have bugs related to database and we compare them with other class files in the commit of database-related issues. First, we calculate the percentage of these two types of class files in all commit files by examining their directory names. Second, we calculate the percentage of database-related issues which have these two types of class files in the commit. Finally, for these two types of class files and other class files, we compare the number of database-related issues related to them. 

%In architecture of database-backed applications, developers maintain persistent objects and database accesses in class files, which are under specific directory. We manually check the applications and Table \ref{tab:database_access_files} gives the result of file directories for persistent object classes and database access classes. For one application, developers follow same rule to name the directory. For example, in subject application BroadleafCommerce, the persistent object classes are located in the directory `/domain' while database access classes in `/dao/'. One persistent object class under the directory `/domain' is `/domain/RoleImpl.java' which is shown in Listing \ref{lst:Snippet_persistent_object}. We can see that this persistent object class handles the entity \textit{role} and maps to the database table \textit{BLC\_ROLE}. Correspondingly, the database access class handling entity \textit{role} is `/dao/RoleDaoImpl.java' under directory `/dao' which is shown in Listing \ref{lst:Snippet_database_access}. The function \textit{readRoleByName} reads entity \textit{role} from database table by name. 

%Thus, we first identify persistent object class files and database access files by their directories, and then measure them on the following metrics:
%\begin{itemize}
%	\item \textbf{Open duration}, which is the amount of time from an issue report is opened to the time when it is fixed. If an issue is difficult to debug and fix, its report would be open for a long time. 
%	
%	\item \textbf{Number of comments}, which counts discussions among developers and users in issue track system for an issue report. More discussions of an issue means that it is more difficult to debug it and more collaborations between participants are needed. 
%	
%	\item \textbf{Number of files changed}, which counts committed files to fix an issue, including added, deleted and modified files. We use this metric to measure the files tainted by the issue as well as the efforts needed to fix the issue. 
%	
%	\item \textbf{Lines of code changed}, which is the lines of code changed to fix an issue, including added, deleted and modified code. Intuitively, more lines of code changed for an issue means that it is more difficult to fix it.
%\end{itemize}

\begin{comment}
\begin{table*}[]
\caption{Medians (Med.) and effect sizes (Eff.) of the metrics for changed files of database-related issues (DBIssue) and non database-related issues (NDBIssue). H: DBIssue $\neq$ NDBIssue, namely alternative = "two.sided" and paired = FALSE, in R}
\label{tab:issues_metric}
\centering
\scalebox{1.0}{
\begin{tabular}{ll|cc|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Metric}} & 
\multirow{2}{*}{\textbf{Type}} & 
\multicolumn{2}{c}{\texttt{\textbf{Broadleaf}}} &
\multicolumn{2}{c}{\texttt{\textbf{metasfresh}}} &
\multicolumn{2}{c}{\texttt{\textbf{Openfire}}}  &
\multicolumn{2}{c}{\texttt{\textbf{adempiere}}} &
\multicolumn{2}{c}{\texttt{\textbf{dbeaver}}} &
\multicolumn{2}{c}{\texttt{\textbf{dotCMS}}} &
\multicolumn{2}{c}{\texttt{\textbf{openmrs}}}

\\\cmidrule(l){3-16} 
&&Med.&p&Med.&p&Med.&p&Med.&p.&Med.&p&Med.&p&Med.&p.\\
\midrule


\tabincell{l}{LOC modified}
&\tabincell{l}{DbIssue\\NDbIssue}  
&\tabincell{l}{28.5\\32.5}&0.91
&\tabincell{l}{ 32 \\ 178.5 }& 0.04
&\tabincell{l}{ 9 \\ 49.5 }& 0.01
&\tabincell{l}{ 24 \\ 41 }& 0.13
&\tabincell{l}{ 15 \\ 12 }& 0.75
&\tabincell{l}{ 20 \\ 34.5 }& 0.57
&\tabincell{l}{ 24 \\ 35 }& 0.10
\\\midrule


\tabincell{l}{Files modified} 
&\tabincell{l}{DbIssue\\NDbIssue} 
&\tabincell{l}{2.5\\2}&0.27
&\tabincell{l}{ 2 \\ 6 }& 0.07
&\tabincell{l}{ 1 \\ 2 }& 0.07
&\tabincell{l}{ 2 \\ 2 }& 0.22
&\tabincell{l}{ 2 \\ 1 }& 0.56
&\tabincell{l}{ 2 \\ 1.5 }& 0.70
&\tabincell{l}{ 3 \\ 3 }& 0.33
\\

\bottomrule
\end{tabular}}
\end{table*}

\begin{table*}[]
\caption{Medians (Med.) and effect sizes (Eff.) of the metrics for changed files of commits between database-related issues (DBIssue) and non database-related issues (NDBIssue). H: DBIssue $\neq$ NDBIssue, namely alternative = "two.sided" and paired = FALSE, in R}
\label{tab:commits_metric}
\centering
\scalebox{1.0}{
\begin{tabular}{ll|cc|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Metric}} & 
\multirow{2}{*}{\textbf{Type}} & 
\multicolumn{2}{c}{\texttt{\textbf{Broadleaf}}} &
\multicolumn{2}{c}{\texttt{\textbf{metasfresh}}} &
\multicolumn{2}{c}{\texttt{\textbf{Openfire}}}  &
\multicolumn{2}{c}{\texttt{\textbf{adempiere}}} &
\multicolumn{2}{c}{\texttt{\textbf{dbeaver}}} &
\multicolumn{2}{c}{\texttt{\textbf{dotCMS}}} &
\multicolumn{2}{c}{\texttt{\textbf{openmrs}}}

\\\cmidrule(l){3-16} 
&&Med.&p&Med.&p&Med.&p&Med.&p.&Med.&p&Med.&p&Med.&p.\\
\midrule

\tabincell{l}{LOC modified}
&\tabincell{l}{DbIssue\\NDbIssue}  
&\tabincell{l}{ 29 \\ 17 }& 0.41
&\tabincell{l}{ 13.5 \\ 19 }& 0.32
&\tabincell{l}{ 10 \\ 28 }& 0.06
&\tabincell{l}{ 13 \\ 28 }& 0.05
&\tabincell{l}{ 15 \\ 10 }& 0.17
&\tabincell{l}{ 16.5 \\ 26 }& 0.31
&\tabincell{l}{ 15 \\ 15 }& 0.32
\\\midrule

\tabincell{l}{Files modified} 
&\tabincell{l}{DbIssue\\NDbIssue} 
&\tabincell{l}{ 2 \\ 1 }& 0.19
&\tabincell{l}{ 1 \\ 1 }& 0.59
&\tabincell{l}{ 1 \\ 1 }& 0.21
&\tabincell{l}{ 1 \\ 1 }& 0.10
&\tabincell{l}{ 1 \\ 1 }& 0.11
&\tabincell{l}{ 1 \\ 1 }& 0.53
&\tabincell{l}{ 1 \\ 1 }& 0.42
\\\midrule

Entropy
&\tabincell{l}{DbIssue\\NDbIssue} 
&\tabincell{l}{ 0.27 \\ 0 }& 0.08
&\tabincell{l}{ 0 \\ 0 }& 0.99
&\tabincell{l}{ 0 \\ 0 }& 0.54
&\tabincell{l}{ 0 \\ 0 }& 0.04
&\tabincell{l}{ 0 \\ 0 }& 0.14
&\tabincell{l}{ 0 \\ 0 }& 0.34
&\tabincell{l}{ 0 \\ 0 }& 0.32
\\
\bottomrule
\end{tabular}}
\end{table*}
\end{comment}

\begin{comment}
\begin{table*}[]
	\caption{\peter{don't just use the union and intersection symbol. If you want to use those symbols, define them. Explain in the caption what they are.}Unique changed files for database-related issues (DBIssue) and non database-related issues (NDBIssue). \peter{also, try to show the percentage of common files across all modified files, we want to show that developers change very different set of files}}
	\label{tab:issues_unique_files}
	\centering
	\scalebox{0.9}{
		\begin{tabular}{ll|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
			\toprule
			\multirow{2}{*}{\textbf{}} & 
			\multirow{2}{*}{\textbf{Type}} & 
			\multicolumn{3}{c}{\texttt{\textbf{Broadleaf}}} &
			\multicolumn{3}{c}{\texttt{\textbf{metasfresh}}} &
			\multicolumn{3}{c}{\texttt{\textbf{Openfire}}}  &
			\multicolumn{3}{c}{\texttt{\textbf{adempiere}}} &
			\multicolumn{3}{c}{\texttt{\textbf{dbeaver}}} &
			\multicolumn{3}{c}{\texttt{\textbf{dotCMS}}} &
			\multicolumn{3}{c}{\texttt{\textbf{openmrs}}}
			
			\\\cmidrule(l){3-23} 
			&&\#&$\cap$&$\cup$&\#&$\cap$&$\cup$&\#&$\cap$&$\cup$&\#&$\cap$&$\cup$&\#&$\cap$&$\cup$&\#&$\cap$&$\cup$&\#&$\cap$&$\cup$\\
			\midrule
			
			
			\tabincell{l}{Unique files \\ modified}
			&\tabincell{l}{DbIssue\\NDbIssue}  
			&\tabincell{l}{110\\68}&17&161
			&\tabincell{l}{62\\262}&7&317 
			&\tabincell{l}{31\\77}&9&99
			&\tabincell{l}{59\\116}&3&172
			&\tabincell{l}{178\\360}&58&480
			&\tabincell{l}{125\\104}&5&224
			&\tabincell{l}{145\\193}&41&297
			\\
			
			\bottomrule
	\end{tabular}}
\end{table*} 
\end{comment}

%Second, we study distribution on the repeated times of commit files for database-related issues.
%Figure \ref{fig_distribution_commit_files_boxplot} shows the distribution. For most commit files, they are committed around 1 $\sim$ 2 times while a few files are committed several times. \wei{Actually, the distribution of commit times between DBIssue and NDBIssue is nearly the same.}
%
%\begin{figure}[ht]
%	\centering
%	\includegraphics[width=\linewidth]{./image/distribution_commit_files_boxplot}
%	\caption{Distribution on the repeated times of committed files for database access bugs across applications.\wei{distribution of commit for DBIusse. We may find that some files are changed more frequently while other files are not frequently changed}}
%	\label{fig_distribution_commit_files_boxplot}
%\end{figure}

%We rank all commit files in ascending order by repeated times and calculate the percentage of repeated times for top N files. Table \ref{tab:percentage_repeated_times} shows the percentage of top N files and Table \ref{tab:repeated_times} shows repeated times of top N files. In average, top \%1, \%5 \%10 and \%15 most repeated files account for \%6, \%16 \%24 and \%32 of all commit files and they are committed 5, 4, 3 and 3 times, respectively. The result shows that some files are changed more frequently to fix the issues and suggests that developers should pay more attention on these files because database-related issues are prone to occur in them. 

%\begin{table}[]
%	\caption{Percentage of top N files}
%	\label{tab:percentage_repeated_times}
%	\begin{tabular}{lcccc}
%		\toprule
%		\multirow{2}{*}{Application} & \multicolumn{3}{c}{Percentage (\%)}   \\\cmidrule(l){2-5} 
%		
%		&Top\%1&Top\%5 &Top\%10 &Top\%15\\
%		\midrule
%		BroadleafCommerce &4	&16    &26    &34\\
%		metasfresh        &5	&10    &17    &24\\
%		Openfire          &9	&22    &30    &37\\
%		adempiere         &5	&15    &23    &31\\   
%		Avg.			  &6	&16    &24    &32\\    
%		\bottomrule
%	\end{tabular}
%\end{table}
%
%\begin{table}[]
%	\caption{Repeated times of top N files}
%	\label{tab:repeated_times}
%	\begin{tabular}{lcccc}
%		\toprule
%		\multirow{2}{*}{Application} & \multicolumn{4}{c}{Repeated Times}   \\\cmidrule(l){2-5} 
%		
%		&Top\%1&Top\%5 &Top\%10 &Top\%15\\
%		\midrule
%		BroadleafCommerce &5.3	&4.3    &3.5    &3\\
%		metasfresh        &4.5	&3.1    &2.5    &2.8\\
%		Openfire          &6	&4.6    &3.8    &3.2\\
%		adempiere         &6 	&4.5    &4.0    &3.7\\   
%		Avg.			  &5	&4    	&3    	&3\\    
%		\bottomrule
%	\end{tabular}
%\end{table}

%\begin{table}[]
%	\caption{Percentage of repeated times for top N files (\%)}
%	\label{tab:percentage_repeated_times}
%	\begin{tabular}{lccccc}
%		\toprule
%		\multirow{2}{*}{Application} & \multicolumn{4}{c}{percentage}   \\\cmidrule(l){2-6} 
%		
%		&Top\%1 &Top\%3 &Top\%5 &Top\%10 &Top\%15 \\
%		\midrule
%		BroadleafCommerce &4	&11	&16     &26    &34    \\
%		metasfresh        &5	&8	&10     &17    &24    \\
%		Openfire          &9	&17	&22    &30     &37    \\
%		adempiere         &5	&8	&15    &23     &31    \\   
%		Avg.			  &6	&11	&16    &24     &32    \\    
%		\bottomrule
%	\end{tabular}
%\end{table}

%\begin{table}[]
%	\caption{percentage of repeated times for top N files (\%)}
%	\label{tab:percentage_repeated_times}
%	\begin{tabular}{lcccc}
%		\toprule
%		\multirow{2}{*}{Application} & \multicolumn{4}{c}{percentage}   \\\cmidrule(l){2-5} 
%		
%		&Top\%5 &Top\%10 &Top\%15 &Top\%20 \\
%		\midrule
%		BroadleafCommerce &16.8     &26.3    &34  	&41.1    \\
%		metasfresh        &10.9     &17.8    &24.7  &31.6                \\
%		Openfire          &22.5    &30.6     &37     &43.5    \\
%		adempiere         &15.1    &23.5     &31  	&36.1    \\     
%		\bottomrule
%	\end{tabular}
%\end{table}

%Second, we study distribution of repeated times for commit files. We rank all commit files in ascending order by repeated times and calculate the percentage of repeated times for top N files. Table \ref{tab:percentage_repeated_times} shows the percentage of top N files and Table \ref{tab:repeated_times} shows repeated times of top N files. In average, top \%1, \%5 \%10 and \%15 most repeated files account for \%6, \%16 \%24 and \%32 of all commit files and they are committed 5, 4, 3 and 3 times, respectively. The result shows that some files are changed more times to fix the issues and suggests that developers could pay more attention on these files because database-related issues are prone to occur in them.

%For example in studied application \texttt{openmrs}, java source code files in directory "\texttt{api/src/main/java/org/openmrs/api/db/}" access the database directly while java source code files in directory "\texttt{api/src/main/java/org/openmrs/}" map to the database tables. 

%Table \ref{tab:percentage_database_access_files} shows the result and in average 30\% of commit files contain persistent object or database access. We also calculate the percentage of database-related issues which have these two types of class files in the commit. Table \ref{tab:percentage_database_related_issues} shows the result and in average 31\% of database-related issues need to fix persistent object or database access class files. This result suggests that nearly 1/3 of database-related issues occur in persistent object or database access class files. However, there are quite a lot of database-related issues only occur in other class files of business source code.

\begin{comment}
\begin{table*}[]
	\caption{Percentage(\%) of issues, commits and files which contain persistent object classes and/or database access classes in database-related issues.\wei{I will check app \texttt{dbeaver} manually. I will only keep the column 'Database access' and other columns are for reviewing.}\wei{some commit files contain database access methods while others do not.}}
	\label{tab:percentage_database_access}
	\centering
	\scalebox{0.9}{
		\begin{tabular}{lccc|ccc|ccc}
			\toprule
			\multirow{3}{*}{\textbf{Application}} & 
			\multicolumn{3}{c}{\textbf{File}} &
			\multicolumn{3}{c}{\textbf{Commit}} &
			\multicolumn{3}{c}{\textbf{Issue}}\\
			\cmidrule(l){2-10} 
			
			&\tabincell{l}{Database\\ access}&\tabincell{l}{Persistent\\ object}&\tabincell{l}{Database access\\Persistent object}
			&\tabincell{l}{Database\\ access}&\tabincell{l}{Persistent\\ object}&\tabincell{l}{Database access\\Persistent object}
			&\tabincell{l}{Database\\ access}&\tabincell{l}{Persistent\\ object}&\tabincell{l}{Database access\\Persistent object}\\
			\midrule
			
			\texttt{BroadleafCommerce}	
			&14.3&31.4&45.7 
			&25.4&28.2&52.1
			&20.4&27.8&44.4
			\\ 
			
			\texttt{metasfresh}  				
			&21.3&9.8&31.1 
			&23.3&20.0&36.7
			&11.5&15.4&23.1
			\\ 
			
			\texttt{Openfire}					
			&21.4&0.0&21.4
			&22.6&0.0&22.6
			&15.4&0.0&15.4
			\\ 
			
			\texttt{adempiere}			
			&20.7&6.9&27.6
			&44.9&14.3&53.1
			&17.5&4.8&19.0
			\\ 
			
			\texttt{dbeaver}				
			&9.2&0.0&9.2  
			&15.4&0.0&15.4
			&16.7&0.0&16.7
			\\  
			
			\texttt{dotCMS/core}			
			&&&  
			&&&
			&&&\\ 
			
			\texttt{openmrs-core}		
			&12.7&5.9&18.6
			&29.6&14.3&37.8
			&23.8&8.8&27.5
			\\ 
			
			\bottomrule
	\end{tabular}}
\end{table*}
\end{comment}

%Most of these source code files for database access bugs are committed 1 to 2 times \wei{Figure \ref{fig_distribution_commit_files_boxplot}} and 
